Evaluating Quantum Optimization for Dynamic Self-Reliant Community Detection

Power grid partitioning is an important requirement for resilient distribution grids. Since electricity production is progressively shifted to the distribution side, dynamic identification of self-reliant grid subsets becomes crucial for operation. This problem can be represented as a modification to the well-known NP-hard Community Detection (CD) problem. We formulate it as a Quadratic Unconstrained Binary Optimization (QUBO) problem suitable for solving using quantum computation{\color{blue}, which is expected to find better-quality partitions faster. The formulation aims to find communities with maximal self-sufficiency and minimal power flowing between them}. To assess quantum optimization for sizeable problems, we apply a hierarchical divisive method that solves sub-problem QUBOs to perform grid bisections. Furthermore, we propose a customization of the Louvain heuristic that includes self-reliance. In the evaluation, we first demonstrate that this problem examines exponential runtime scaling classically. Then, using different IEEE power system test cases, we benchmark the solution quality for multiple approaches: D-Wave's hybrid quantum-classical solvers, classical heuristics, and a branch-and-bound solver. As a result, we observe that the hybrid solvers provide very promising results, both with and without the divisive algorithm, regarding solution quality achieved within a given time frame. Directly utilizing D-Wave's Quantum Annealing (QA) hardware shows inferior partitioning.

==> sections/old_01_introduction.tex <==
\section{Introduction}\label{sec:introduction}

In the past years, the computing landscape has shifted with the emergence of Quantum Computing (QC) technologies. While quantum computing is still in its infancy, notable development advancements have incited the exploration of potential applications. As one possible field, quantum optimization promises to revolutionize our approach to solving complex computational problems~\cite{abbas2023}.

The expectation of QC to speed up optimization tasks stems from the inherent quantum mechanical properties, superposition, entanglement, and an exponentially growing state space. Grover's algorithm~\cite{grover1996} is one of the first quantum algorithms that exhibits a scaling advantage compared to classical search algorithms. Although equipped with a mathematically proven speedup, the practical use of Grover is still not possible due to the Noisy Intermediate Scale Quantum (NISQ) hardware and the relatively deep circuits involved~\cite{wang2020}.
Instead, short, variational circuits, like the Quantum Approximate Optimization Ansatz (QAOA)~\cite{farhi2014, hadfield2019} or the Variational Quantum Eigensolver (VQE), are the focus of current-day research on quantum optimization applications, with the hope of tapping into quantum advantage as soon as possible. Besides optimization algorithms on universal quantum computers, purpose-built Quantum Annealing (QA) devices for optimization have emerged~\cite{farhi2001, rajak2023}. They rely on the adiabatic principle of quantum mechanics that states if a system evolves slowly enough, the system stays in the ground state of the momentary Hamiltonian~\cite{born1928, farhi2001}.  In that sense, a QA device is initialized with an easily preparable ground state. Subsequently, the system undergoes a gradual transition to a Hamiltonian, where the ground state of the system encodes the solution to a specific optimization problem. Finally, the solution is obtained by measuring the system. Currently, available QA hardware is provided by the company D-Wave and features the usage of quadratically interacting Ising problem Hamiltonians~\cite{mcgeochb}. This problem specification is isomorphic to the Quadratic Unconstrained Binary Optimization (QUBO) problem, in which many NP-complete and NP-hard problems can be formulated~\cite{lucas2014b}.

The application of QA in various domain-specific application tasks, like logistics~\cite{feld2019, weinberg2023, clark2019}, finance~\cite{phillipson2021, lang2022, sakuler2023}, or energy systems~\cite{omeara2023, fernandez-campoamor2021b, halffmann2023, bucher2023}, has been widely explored in literature. In this paper, we will investigate the applicability and benchmark the performance of QA on the task of dynamically identifying microgrids based on momentary loads and production capacities. The use-case is based on a well-known NP-hard optimization problem called Modularity-based Community Detection (CD)~\cite{nadakuditi2012, brandes2006}, which has also been studied in the context of QA~\cite{reittu2019, shaydulin2019a, negre2020a,gemeinhardt2021a, stein2023}. However, we extend the formulation to Self-Reliant Community Detection (SRCD), where the identified microgrids should be mostly self-sustainable. Our benchmarking involves D-Wave's Leap as a hybrid quantum-classical method~\cite{d-wave2021}, Gurobi as a classical mixed-integer branch-and-bound solver~\cite{gurobi}, Simulated Annealing (SA) and QBsolv~\cite{kirkpatrick1983} as classical QUBO heuristics, Louvain's algorithm~\cite{blondel2008} as a classical CD heuristic, and a divisive heuristic that iteratively splits the power grid, allowing for the solution of sub-problems on D-Wave's QA chip. Despite hyperparameter tuning, we observe that the results obtained from the Quantum Processing Unit (QPU) are considerably worse in comparison to the other methods, due to the error-prone hardware.
The application of QA in various domain-specific application tasks, like logistics~\cite{feld2019, weinberg2023, clark2019}, finance~\cite{phillipson2021, lang2022, sakuler2023}, or energy systems~\cite{omeara2023, fernandez-campoamor2021b, halffmann2023, bucher2023}, has been widely explored in literature. In this paper, we will investigate the applicability and benchmark the performance of QA on the task of dynamically identifying microgrids based on momentary loads and production capacities. The use-case is based on a well-known NP-hard optimization problem called Modularity-based Community Detection (CD)~\cite{nadakuditi2012, brandes2006}, which has also been studied in the context of QA~\cite{reittu2019, shaydulin2019a, negre2020a,gemeinhardt2021a, stein2023}. However, we extend the formulation to Self-Reliant Community Detection (SRCD), where the identified microgrids should be mostly self-sustainable. Our benchmarking involves D-Wave's Leap as a hybrid quantum-classical method~\cite{d-wave2021}, Gurobi as a classical mixed-integer branch-and-bound solver~\cite{gurobi}, Simulated Annealing (SA) and QBsolv~\cite{kirkpatrick1983} as classical QUBO heuristics, Louvain's algorithm~\cite{blondel2008} as a classical CD heuristic, and a divisive heuristic that iteratively splits the power grid, allowing for the solution of sub-problems on D-Wave's QA chip. Despite hyperparameter tuning, we observe that the results obtained from the Quantum Processing Unit (QPU) are considerably worse in comparison to the other methods, due to the error-prone hardware.

Microgrids are expected to be one of the core building blocks for a future smart and decentralized power grid~\cite{hirsch2018, oneill2022}. Instead of a centralized power source that gets distributed outwards to the individual customers, the individual customers become generators themselves through installed photovoltaic panels, home battery storage, or vehicle-to-grid technology. The identification of self-sustaining microgrids in such a grid can help the energy operator to install pricing zones for especially self-sustaining parts, financially motivating customers to participate in such a system. Furthermore, microgrids can help the formation of peer-to-peer electricity trading~\cite{bukar2023, omeara2023} since the number of matching partners gets reduced, and the matching within a self-sustained microgrid guarantees that the trade occurs where the physical power is flowing.

The remaining text is structured as follows: We present the mathematical formulation of the SRCD model in Sec.~\ref{sec:formulation}. After that, we will discuss the used solvers in Sec.~\ref{sec:methods} including the adaptation needed for the Louvain algorithm. There, we will also discuss the divisive heuristic and how the sub-problems for it are generated. Sec.~\ref{sec:evaluation} explains the methodology employed for evaluating the performance of the solvers, and Sec.~\ref{sec:results} presents the results of the benchmarks. Finally, we conclude our findings in Sec.~\ref{sec:conclusion}.
